Cloaker Catcher: A Client-based Cloaking Detection System

Cloaking has long been exploited by spammers for the purpose of increasing the exposure of their websites. In other words, cloaking has long served as a major malicious technique in search engine optimization (SEO). Cloaking hides the true nature of a website by delivering blatantly different content to users versus web crawlers. Recently, we have also witnessed a rising trend of employing cloaking in search engine marketing (SEM). However, detecting cloaking is challenging. Existing approaches cannot detect IP cloaking and are not suitable for detecting cloaking in SEM because their search-and-visit method leads to click fraud. In addition, they focus on detecting and measuring cloaking on the server side, but the results are not visible to users to help them avoid frauds. Our work focuses on mitigating IP cloaking and SEM cloaking, and providing client-based real-time cloaking detection services. To achieve these goals, we first propose the Simhash-based Website Model (SWM), a condensed representation of websites, which can model natural page dynamics. Based on SWM, we design and implement Cloaker Catcher, an accurate, efficient and privacy-preserving system, that consists of a server that crawls websites visited by users on demand and a client-side extension that fetches spider views of websites from the server and compares them with user views to detect cloaking. Since Cloaker Catcher checks on the client side for each real user, IP cloaking can be detected whenever it occurs and click fraud in SEM can also be prevented. Using our system, we conducted the first analysis of SEM cloaking and found that the main purpose of SEM cloakers is to provide illicit services.

==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}


==> discussion.tex <==
\section{Limitations}
\label{s:limitation}
%\textbf{Assumptions about visited lists.}
%Incentive analysis is not automatically. Machine learning algorithms to classify.
\textbf{Visibility in SEM.}
While we do measure the cloaking state of SEM, we are still automating browsers to collect user views. This approach has two problems in practice: (A) It is considered as click fraud and is blocked by some security services or tools which fingerprint browsers and IPs of click bots.
(B) Attackers may be aware of us and have blocked all the IPs that we have access to, since we are crawling on a large scale.
Deployment of Cloaker Catcher on real clients can address this visibility issue, and we leave it for future work.

\textbf{False positives.}


\textbf{Incentive analysis automation.}
We manually classify the incentives of cloaking websites in this work. However, according to our observations, this process can be automated using machine learning approaches. For example, cloaking sites that simply embed an iframe is targeting traffic sale, and ones that stays on a domain for a while and redirects users to downloads are doing unwanted software download.

\textbf{Domain features.}
Domain and content are commonly used features in search engine spam detection.
Previous works ~\cite{lu2011surf,leontiadis2014nearly} have used domain related information to detect search engine poisoning. Integrating these two sets of features can improve the detection accuracy. We don't go deep into this because this is not the main contribution of this paper. 

\subsection{False Positive Analysis}

There are mainly two kinds of false positive in SEM. Optimized for different version. (mobile versus desktop). Page load incomplete (doesn't count). Page visit blocked (This page needs more care, common error pages).
Add many advertisements in users' view, but nothing in Googles' view.
%\subsection{SWM Availability at Server side}
%Cloaker Catcher includes a server that periodically crawl websites and build SWM. However, this is a huge amount of work as the number of users increases and become infeasible for individual researchers. Therefore, we advise search engines to adopt our prototype. For individual researchers,
%a trade-off is to periodically since it is not feasible to crawl all the websites and thus we could just periodically crawl words or links that we are interested in, and return not cloaking for unknown URLs.


==> fig/para-select.tex <==
\begin{tabular}{lllllllllll}
  \toprule
  & \multicolumn{2}{c}{\textbf{Normal}}
  & \multicolumn{2}{c}{\textbf{Lognormal}}
  & \multicolumn{2}{c}{\textbf{Exponential}}
  & \multicolumn{2}{c}{\textbf{Gamma}}
  & \multicolumn{2}{c}{\textbf{Logistic}}\\

  \textbf{Website(Hash Type)\textbackslash Model}
  & AD-value
  & P-value
  & AD-value
  & P-value
  & AD-value
  & P-value
  & AD-value
  & P-value
  & AD-value
  & P-value \\
  \midrule
  digg.com T & 0.617 &  0.100 & 0.481 &  0.219 &
  14.851 & < 0.003 & 0.538 &  0.186 & 0.531 &  0.131\\ 
  digg.com T & 0.227 &  0.806 & 0.179 &  0.914 &
  19.690 &  < 0.003 & 0.198 &  > 0.250 & 0.250 & >0.250\\
  yahoo.com T & 0.192 &  0.893 & 0.263 &  0.692 &
  35.828 & <0.003 &   0.231 & >0.250 & 0.222 & >0.250\\
  amazon.com T & 0.720 &  0.058 & 0.323 &  0.520 & 
  27.754 & <0.003 &  0.436 & >0.250 & 0.642 &  0.058\\
  reddit.com T & 0.373 &  0.411 & 0.331  & 0.509 & 
  35.063 & <0.003 & 0.340 & >0.250 & 0.361 & >0.250\\
  yacombinator.com T & 0.473 &  0.237 & 0.516 &  0.186 &
  37.551 & <0.003 & 0.519 &  0.204 & 0.583 &  0.089\\

  digg.com D & 0.319 &  0.372 & 0.348 &  0.305 &
  1.491 &  0.021 &  0.402 & >0.250 & 0.363 & >0.250\\
  yahoo.com D & 0.531 &  0.168 & 0.392 &  0.366 &
  18.837 & <0.003 & 0.441 & >0.250 & 0.584  & 0.088\\
  amazon.com D & 1.519 & <0.005 & 0.916 &  0.019 &
  22.083 & <0.003 & 1.052 &  0.009 & 0.548 &  0.114\\
  amazon.com D & 0.483 & 0.117 &  0.504 & 0.104 &
  1.741 & 0.010 & 0.601 & 0.128 & 0.523 & 0.115\\

\end{tabular}


